Multi-task Hierarchical Adversarial Inverse Reinforcement Learning

Multi-task Imitation Learning (MIL) aims to train a policy capable of performing a distribution of tasks based on multi-task expert demonstrations, which is essential for general-purpose robots. Existing MIL algorithms suffer from low data efficiency and poor performance on complex long-horizontal tasks. We develop Multi-task Hierarchical Adversarial Inverse Reinforcement Learning (MH-AIRL) to learn hierarchically-structured multi-task policies, which is more beneficial for compositional tasks with long horizons and has higher expert data efficiency through identifying and transferring reusable basic skills across tasks. To realize this, MH-AIRL effectively synthesizes context-based multi-task learning, AIRL (an IL approach), and hierarchical policy learning. Further, MH-AIRL can be adopted to demonstrations without the task or skill annotations (i.e., state-action pairs only) which are more accessible in practice. Theoretical justifications are provided for each module of MH-AIRL, and evaluations on challenging multi-task settings demonstrate superior performance and transferability of the multi-task policies learned with MH-AIRL as compared to SOTA MIL baselines.

==> background_full.tex <==
\section{Background and Related Works}

In this section, we introduce the background on Adversarial Inverse Reinforcement Learning (AIRL), Context-based Meta Learning, and the One-step Option Framework, corresponding to the three components of our algorithm: IL, context-based multi-task learning, and hierarchical policy learning, respectively.  They are defined based on the Markov Decision Process (MDP), denoted by $\mathcal{M}=(\mathcal{S}, \mathcal{A}, \mathcal{P}, \mu, \mathcal{R}, \mathcal{\gamma})$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}:\mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow [0,1]$ is the state transition function ($\mathcal{P}^{S_{t+1}}_{S_{t}, A_{t}}\triangleq\mathcal{P}(S_{t+1}|S_{t}, A_{t})$), $\mu:\mathcal{S}\rightarrow [0,1]$ is the distribution of the initial state, $\mathcal{R}:\mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function, and $\mathcal{\gamma} \in (0,1]$ is the discount factor. 

\subsection{Adversarial Inverse Reinforcement Learning} \label{airl}

While there are several other ways to perform Imitation Learning, such as supervised imitation (e.g., Behavioral Cloning (BC) \cite{DBLP:journals/neco/Pomerleau91}) and occupancy matching (e.g., GAIL \cite{DBLP:conf/nips/HoE16}), we adopt Inverse Reinforcement Learning (IRL) \cite{DBLP:conf/icml/NgR00} because it's not only based on the expert data but also makes use of the self-exploration of the agent with the recovered reward function. We compare our IRL-based algorithm with BC- and GAIL-based algorithms in the evaluations.
 
 IRL aims to infer an expert's reward function from demonstrations, based on which the policy of the expert can be recovered. As a representative, Maximum Entropy IRL \cite{DBLP:conf/aaai/ZiebartMBD08} solves it as a maximum likelihood estimation (MLE) problem shown as Equation \ref{equ:1} and \ref{equ:2}. $\tau_{E}\triangleq (S_0, A_0, \cdots, S_T)$ denotes the expert trajectory, i.e., a sequence of state-action pairs of horizon $T$. $Z_{\vartheta}$ is the partition function which can be calculated with $Z_{\vartheta}=\int\widehat{P}_{\vartheta}(\tau_{E})d\tau_{E}$ (continuous $\mathcal{S}$ and $\mathcal{A}$) or $Z_{\vartheta}=\sum_{\tau_{E}}\widehat{P}_{\vartheta}(\tau_{E})$ (discrete $\mathcal{S}$ and $\mathcal{A}$).
\begin{equation} \label{equ:1}
    \mathop{max}_{\vartheta}\mathbb{E}_{\tau_{E}}\left[logP_{\vartheta}(\tau_{E})\right]=\mathbb{E}_{\tau_{E}}\left[log\frac{\widehat{P}_{\vartheta}(\tau_{E})}{Z_{\vartheta}}\right]
\end{equation}
\begin{equation} \label{equ:2}
    \widehat{P}_{\vartheta}(\tau_{E})=\mu(S_0)\mathop{\prod}_{t=0}^{T-1}\mathcal{P}^{S_{t+1}}_{S_{t}, A_{t}}exp(\mathcal{R}_{\vartheta}(S_t, A_t))
\end{equation}

Since $Z_{\vartheta}$ is intractable for the large-scale state-action space, the authors of \cite{DBLP:journals/corr/abs-1710-11248} propose Adversarial Inverse Reinforcement Learning (AIRL) to solve this MLE problem in a sample-based manner. They realize this through alternatively training a discriminator $D_{\vartheta}$ and policy network $\pi$ in an adversarial setting. Specifically, the discriminator is trained by minimizing the cross-entropy loss between the expert demonstrations $\tau_{E}$ and generated samples $\tau$ by $\pi$:
\begin{equation} \label{equ:3}
\begin{aligned}
    \mathop{min}_{\vartheta}\mathop{\sum}_{t=0}^{T-1}-\mathbb{E}_{\tau_{E}}\left[logD_{\vartheta}(S_t,A_t)\right]  - \mathbb{E}_{\tau}\left[log(1-D_{\vartheta}(S_t,A_t))\right]
\end{aligned}
\end{equation}
where $D_{\vartheta}(S,A)=\frac{exp(f_{\vartheta}(S,A))}{exp(f_{\vartheta}(S,A))+\pi(A|S)}$. Meanwhile, the policy $\pi$ is trained with off-the-shelf RL algorithms using the reward function defined as $logD_{\vartheta}(S,A)-log(1-D_{\vartheta}(S,A))$. Further, they justify that, at optimality, $f_{\vartheta}(S,A)$ can serve as the recovered reward function $\mathcal{R}_{\vartheta}(S,A)$ and $\pi$ is the recovered expert policy which maximizes the entropy-regularized objective: $\mathbb{E}_{\tau \sim \pi}\left[\mathop{\sum}_{t=0}^{T-1}\mathcal{R}_{\vartheta}(S_t,A_t)-log\pi(A_t|S_t)\right]$.


\subsection{Context-based Meta Learning} \label{context}

% Meta Learning, also known as learning to learn, seeks to exploit the structural similarity among a distribution of tasks and optimizes for rapid adaptation to unknown settings with a limited amount of data. 
We consider the Meta RL/IRL setting: given a distribution of tasks $P(\mathcal{T})$, each task sampled from $P(\mathcal{T})$ has a corresponding MDP, and all of them share the same state and action space but may differ in the initial state distribution, reward function and transition dynamics. The goal is to train a flexible policy $\pi$ on a set of training tasks sampled from $P(\mathcal{T})$, which can be quickly adapted to unseen test tasks sampled from the same distribution. As a representative, context-based Meta RL/IRL algorithms \cite{DBLP:conf/icml/RakellyZFLQ19, DBLP:conf/nips/GhasemipourGZ19, DBLP:conf/nips/YuYFE19} introduce the latent task variable $C$ which provides an abstraction of the corresponding task $\mathcal{T}$. Thus, the distinctive components of each task are additionally conditioned on its corresponding $C$, i.e., $\{\mu(S_0|C), \mathcal{P}(S'|S,A,C), \mathcal{R}(S,A|C)\}$. These algorithms train a task inference model $P(C|\mathcal{T})$ and a policy agent $\pi(A|S,C)$ in the meanwhile so that, when met with a new test task, the agent can first infer the task latent $C$ based on the experience and then apply the corresponding policy $\pi(A|S,C)$ to realize a fast adaption. If $C$ is given as a prior, they can directly use $\pi(A|S,C)$ for the task without further adaption. Context-based methods can adopt off-policy data, which makes them more sample-efficient than the gradient-based Meta Learning methods \cite{DBLP:conf/cogsci/WangKSLTMBKB17, finn2017model, DBLP:conf/iclr/RothfussLCAA19} and in accord with the goal of our work -- learning from demonstrations. Thus, we choose context-based Meta IRL as our base algorithm.

% As mentioned in Section \ref{airl}, IRL can be adopted to recover the expert's reward function and policy from a set of demonstrations. While, for context-based Meta IRL \cite{DBLP:conf/nips/GhasemipourGZ19, DBLP:conf/nips/YuYFE19}, the goal is to learn a task inference model $P_{\omega}(C|\tau)$ and recover the task-conditioned reward function $\mathcal{R}_{\vartheta}(S,A|C)$ and policy $\pi(S,A|C)$, given a mixture of expert trajectories sampled from multiple tasks. 
% learn a task inference model $P_{\omega}(C|\tau)$,
Given a mixture of expert trajectories sampled from multiple tasks, context-based Meta IRL needs to recover the task-conditioned reward function $\mathcal{R}_{\vartheta}(S,A|C)$ and policy $\pi(S,A|C)$. 
% It's assumed that the expert trajectories follow the distribution $P(\tau_{E})=\sum_{\mathcal{C}}P^{prior}(C)\pi_{E}(\tau_{E}|C)$ or $P(\tau_{E})=\int_{\mathcal{C}}P^{prior}(C)\pi_{E}(\tau_{E}|C)dC$, where $\mathcal{C}$ denotes the task latent space which can be discrete or continuous. 
It is assumed that the multiple tasks follow the same distribution $prior(C)$ and the demonstrative trajectories of each task are sampled from a corresponding expert policy $\pi_{E}(\tau_{E}|C)$. 
% When dealing with a new task, the agent can infer the latent variable based on few demonstrations from the task using $P_{\omega}(C|\tau)$, and then adopt the corresponding $\pi(S,A|C)$ directly for testing. 
The task-conditioned reward function and policy can be recovered by solving an MLE problem:
\begin{equation} \label{equ:6}
\begin{aligned}
        &\ \ \ \ \ \mathop{max}_{\vartheta}\mathbb{E}_{C\sim prior(\cdot),\tau_{E} \sim \pi_{E}(\cdot|C)}\left[logP_{\vartheta}(\tau_{E}|C)\right],\\
    &P_{\vartheta}(\tau_{E}|C)\propto \mu(S_0|C)\prod_{t=0}^{T-1}\mathcal{P}^{S_{t+1}}_{S_{t}, A_{t}, C}\ e^{\mathcal{R}_{\vartheta}(S_t, A_t|C)}
\end{aligned}
\end{equation}
where $\mathcal{P}^{S_{t+1}}_{S_{t}, A_{t}, C}\triangleq\mathcal{P}(S_{t+1}|S_{t}, A_{t}, C)$.
Thus, for each specific $C$, this is a Maximum Entropy IRL problem (Equation \ref{equ:1} and \ref{equ:2}) which can be efficiently solved through AIRL. We provide the AIRL framework to solve Equation \ref{equ:6} in Appendix \ref{c-airl}. 

% On the other hand, in \cite{DBLP:conf/nips/YuYFE19}, the task inference model $P_{\omega}(C|\tau)$ is trained as a variational posterior distribution by maximizing the mutual information \cite{cover1999elements} between the task latent $C$ and the trajectory sampled in the corresponding task, i.e., $I(C;\tau)$. We also adopt this idea in our algorithm, which is further discussed in Section \ref{info}.

\subsection{One-step Option Framework} \label{option}

% Temporal abstraction allows representing knowledge about courses of action at different time scales, which is key to scaling up learning and planning in RL. The temporal abstraction in RL can be modeled with the option framework proposed in \cite{DBLP:journals/ai/SuttonPS99}.

As proposed in \cite{DBLP:journals/ai/SuttonPS99}, an option $Z \in \mathcal{Z}$ can be described with three components: an initiation set $I_Z \subseteq \mathcal{S}$, an intra-option policy $\pi_Z(A|S): \mathcal{S} \times \mathcal{A} \rightarrow [0,1]$, and a termination function $ \beta_Z(S): \mathcal{S} \rightarrow [0,1]$. An option $Z$ is available in state $S$ if and only if $S \in I_Z$. Once the option is taken, actions are selected according to $\pi_Z$ until it terminates stochastically according to $\beta_Z$, i.e., the termination probability at the current state. A new option will be activated by a high-level policy $\pi_\mathcal{Z}(Z|S): \mathcal{S} \times \mathcal{Z} \rightarrow [0,1]$ once the last option terminates. In this way, $\pi_\mathcal{Z}(Z|S)$ and $\pi_Z(A|S)$ constitute a hierarchical policy for a certain task. Hierarchical policies tend to have superior performance on long-horizontal, complex tasks, which can often be
broken down and processed as a series of subtasks.

The one-step option framework \cite{DBLP:conf/nips/ZhangW19a, DBLP:conf/icml/JingH0MKGL21} is proposed to learn the hierarchical policy without the extra need to justify the exact beginning and breaking condition of each option, i.e., $I_Z$ and $\beta_Z$. It's assumed that each option is available in each state, i.e., $I_Z=\mathcal{S}, \forall Z \in \mathcal{Z}$. Also, the high-level and low-level (i.e., intra-option) policy are redefined as $\pi_{\theta}$ and $\pi_{\phi}$ respectively:
\begin{equation} \label{equ:4}
\begin{aligned}
    \pi_{\theta}(Z|S, Z')=&\beta_{Z'}(S)\pi_{\mathcal{Z}}(Z|S) + (1-\beta_{Z'}(S))\mathbbm{1}_{Z=Z'},\\ &\pi_{\phi}(A|S,Z)=\pi_Z(A|S)
\end{aligned}
\end{equation}
where $Z'$ denotes the option in the last time step and $\mathbbm{1}_{Z=Z'}$ is the indicator function. The option is selected at each step -- if the previous option terminates (with probability $\beta_{Z'}(S)$), the agent will select a new option according to $\pi_{\mathcal{Z}}(Z|S)$; otherwise, it will stick to $Z'$. Nevertheless, $\pi_{\theta}(Z|S, Z')$ still includes two separate parts, i.e., $\beta_{Z'}(S)$ and $\pi_{\mathcal{Z}}(Z|S)$, and due to the indicator function, the update gradients of $\pi_{\mathcal{Z}}$ will be blocked/gated by the termination function $\beta_{Z'}(S)$. In this case, the authors of \cite{li2020skill} propose to marginalize the termination function away, and instead implement $\pi_{\theta}(Z|S, Z')$ as an end-to-end neural network (NN) with the Multi-Head Attention (MHA) mechanism \cite{DBLP:conf/nips/VaswaniSPUJGKP17} which enables their algorithm to temporally extend options in the absence of the termination function. With the marginalized one-step option framework, we only need to learn the two NN-based policies, i.e., $\pi_{\theta}$ and $\pi_{\phi}$, and we give out an actor-critic algorithm for updating the policies in Section \ref{frame}.  We provide the structure design of $\pi_{\theta}$ and $\pi_{\phi}$ with MHA in Appendix \ref{mha}.

==> evaluation_full.tex <==


\section{Evaluation and Main Results}

MH-AIRL is proposed to learn a multi-task hierarchical policy from a mixture of (unstructured) expert demonstrations. The learned policy can be adopted to any task sampled from a distribution of tasks. This section focuses on: (1) Our algorithm has three main components: context-based multi-task/meta learning, option/hierarchical learning, and imitation learning. We will show the necessity of each algorithm module through an ablation study. (2) We will evaluate whether the hierarchical policy learning (i.e., the introduction of the option framework) can significantly improve the agent's performance on challenging long-horizontal tasks. (3) Through qualitative and quantitative results, we will explore whether our algorithm can capture the subtask structure within the expert demonstrations and whether the learned basic skills for the subtasks (i.e., options) can be transferred to tasks not within the class to aid learning so that the transferability of the learned multi-task policy can be improved.

The evaluation is based on three Mujoco \cite{todorov2012mujoco} locomotion tasks and the Kitchen task from the D4RL benchmark \cite{DBLP:journals/corr/abs-2004-07219}. All of them are continuous control tasks with continuous state \& action spaces, and contain compositional subtask structures to make them long-horizontal and a lot more challenging. To be specific: (1) In \textbf{HalfCheetah-MultiVel}, the goal velocity $v$ is controlled by a 1-dim Gaussian context variable. The HalfCheetah agent is required to speed up to $v/2$ first, then slow down to 0, and finally achieve $v$. (2) In \textbf{Walker-RandParam}, the Walker agent must achieve the goal velocity 4 in three stages, i.e., [2, 0, 4]. Meanwhile, the mass of the agent changes among different tasks, which is controlled by a 8-dim Gaussian context variable. (3) In \textbf{Ant-MultiGoal}, a 3D Ant agent needs to reach a certain goal, which is different in each task and controlled by a 2-dim Gaussian context variable (polar coordinates). Moreover, the agent must go through certain subgoals. For example, if the goal is $(x, y)$ and $|x|>|y|$, the agent must go along $[(0, 0), (x, 0), (x, y)]$. (4) In \textbf{Kitchen-MultiSeq}, there are seven different subtasks, like manipulating the microwave, kettle, cabinet, switch, burner, etc, in the same kitchen environment. The accomplishment of each task requires sequentially completions of four specific subtasks out of those seven. Twenty-four permutations are chosen and so 24 tasks, each of which is sampled with the same probability and controlled by a discrete context variable (input as one-hot vectors). Note that the states of the robot agents only contain their original states (defined by Mujoco or D4RL) and the task context variable, and do not include the actual task information, like the goal (velocity) and subgoal list, which is more challenging and makes our algorithm more general. 

These scenarios are designed to evaluate our algorithm on a wide range of multi-task setups. First, the agent needs to adapt across different reward functions in (1)(3) since the rewarding state changes, and adjust across different transition functions in (2) since the mass change will influence the robotic dynamics. Next, different from (1)-(3), discrete context variables are adopted in (4), and (4) provides more realistic and challenging robotic tasks to test on.

The expert data for the Mujoco tasks are from expert agents trained with a Hierarchical RL algorithm \cite{DBLP:conf/nips/ZhangW19a} and specifically-designed reward signals. While, for the Kitchen task, we use the human demonstrations provided by \cite{DBLP:conf/corl/0004KLLH19}. Note that the demonstrations do not include the rewards, task or option contexts. The codes for reproducing all the results are on \href{https://anonymous.4open.science/r/MH-AIRL}{https://anonymous.4open.science/r/MH-AIRL}.

\begin{table*}[t]
\centering
\caption{Numeric results of the ablation study}
\begin{tabular}{c || c c c c}
\hline
{ } & {HalfCheetah-MultiVel} & {Walker-RandParam} & {Ant-MultiGoal} & {Kitchen-MultiSeq}\\
\hline
\hline
{Expert} & {$376.55 \pm 11.12$} & {$399.95 \pm 1.43$} & {$1593.17 \pm 40.91$} & {$400.00 \pm 0.00$}\\
\hline
{MH-AIRL (ours)} & {\bm{$292.79 \pm 15.99$}} & {\bm{$357.59 \pm 12.10$}} & {\bm{$1530.82 \pm 15.18$}} & {\bm{$352.59 \pm 15.12$}}\\
\hline
\makecell[c]{MH-GAIL (ours)}
 & {$211.32 \pm 52.74$} & {$268.92 \pm 49.29$} & {$1064.78 \pm 180.28$} & {$212.13 \pm 25.25$} \\  
\hline
\makecell[c]{H-AIRL (ours)}
 & {$126.85 \pm 21.92$} & {$225.48 \pm 12.87$} & {$533.80 \pm 40.69$} & {$83.97 \pm 10.95$} \\  
\hline
\makecell[c]{Option-GAIL}
 & {$-44.89 \pm 51.95$} & {$132.01 \pm 54.75$} & {$383.05 \pm 13.52$} & {$204.73 \pm 56.41$} \\  
\hline
\makecell[c]{DI-GAIL}
 & {$56.77 \pm 49.76$} & {$225.22 \pm 14.01$} & {$328.06 \pm 19.89$} & {$131.79 \pm 53.29$} \\  
\hline
\end{tabular}
\label{table:1}
\end{table*}

\begin{figure*}[t]
\centering
\subfigure[PointCell-MultiGoal]{
\label{fig:6(a)} 
\includegraphics[width=1.8in, height=1.2in]{figs/PointCell_env.eps}}
\subfigure[PointRoom]{
\label{fig:6(b)} 
\includegraphics[width=1.8in, height=1.2in]{figs/PointRoom_env.eps}}
\subfigure[PointMaze]{
\label{fig:6(c)} 
\includegraphics[width=1.8in, height=1.2in]{figs/PointMaze_env.eps}}
\subfigure[Recovered Hier Policy]{
\label{fig:6(d)} 
\includegraphics[width=1.4in, height=1.2in]{figs/point_trajs.eps}}
\subfigure[Transfer Learning on PointRoom]{
\label{fig:6(e)} 
\includegraphics[width=2.0in, height=1.2in]{figs/PointRoom.eps}}
\subfigure[Transfer Learning on PointMaze]{
\label{fig:6(f)} 
\includegraphics[width=2.0in, height=1.2in]{figs/PointMaze.eps}}
\caption{(a) The environment for multi-task learning with MH-AIRL. (b)(c) New task settings for evaluating the learned options in (a). (d) The trajectories of the learned hierarchical policy, where different options are labeled with different colors and each of the automatically-discovered options corresponds to a particular forward direction. (e)(f) Comparison results between our proposed HRL algorithm (i.e., HPPO) initialized with the transferred options (i.e., HPPO-init) and other SOTA HRL and RL baselines.}
\label{fig:6} 
\end{figure*}

\subsection{Effect of Hierarchical Learning} \label{ehl}

In this part, we evaluate whether the use of the option framework can significantly improve the learning for challenging compound multi-task settings introduced above. We compare our algorithm (MH-AIRL) with state-of-the-art (SOTA) Meta Imitation Learning (MIL) baselines which also aim to train a policy that can be fast adapted to a class of related tasks but do not adopt options in the learning process. Context-based MIL, such as \textbf{PEMIRL} \cite{DBLP:conf/nips/YuYFE19} and \textbf{SMILE} \cite{DBLP:conf/nips/GhasemipourGZ19}, learns a context-conditioned policy that can be adopted to any task from a class by applying the task context. While, the policy learned with Gradient-based MIL, such as \textbf{MAML-IL} \cite{DBLP:conf/corl/FinnYZAL17} which integrates MAML \cite{DBLP:conf/icml/FinnAL17}, a commonly-adopted Meta Learning algorithm, and Behavioral Cloning (BC), has to be updated with gradients calculated based on trajectories from the new task, before being applied. We select PEMIRL, SMILE, and MAML-IL from the two major categories of MIL as our baselines. All the algorithms are trained with the same expert data, and evaluated on the same set of test tasks which are not contained in the expert demonstrations. Note that, unlike the others, MAML-IL requires expert data of each test task besides the task context variable when testing and requires the expert demonstrations to be categorized by the task when training, which may limit its use in real-life scenarios. Our algorithm is trained based on unstructured demonstrations and is only provided the task context variable for testing.

In Figure \ref{fig:4}, we record the change of the episodic reward (i.e., the sum of rewards for each step in an episode) on the test tasks as the number of training samples increases in the training process for each algorithm. The training is repeated for 5 times with different random seeds for each algorithm, of which the mean and standard deviation are shown as the solid line and shadow area, respectively, so are the following quantitative results. It can be observed that our algorithm outperforms the baselines in the tasks, and the improvement is more and more significant as the task difficulty goes up (e.g., Ant \& Kitchen), which shows the effectiveness of hierarchical policy learning especially in complex tasks. MAML-IL makes use of more expert information in both training and testing, but its performance gets worse on more challenging tasks. This may be because it is based on BC, which is a supervised learning algorithm and prone to compounding errors \cite{DBLP:journals/jmlr/RossGB11} in cases that the demonstrations are not sufficient for complex settings.

\begin{figure*}[t]
\centering
\subfigure[Results on HalfCheetah-MultiVel]{
\label{fig:7(a)} 
\includegraphics[width=4.0in, height=1.2in]{figs/Visual_HalfCheetah.eps}}
\subfigure[Results on Walker-RandParam]{
\label{fig:7(b)} 
\includegraphics[width=2.0in, height=1.2in]{figs/Visual_Walker.eps}}
\caption{(a) Velocity change of the HalfCheetah agent in the test tasks with different goal velocities, where the agent adopts Option 1 (blue) and 2 (orange) when increasing and decreasing the speed, respectively. (b) For Walker-RandParam, the basic skills must adapt to the task setting, so the learning performance would drop without conditioning the low-level policy (i.e., option) on the task context.}
\label{fig:7} 
\end{figure*}

% \begin{figure}[t]
% \centering
% \includegraphics[width=3.0in, height=1.3in]{figs/Visual_HalfCheetah.eps}
% % \includegraphics[width=3.0in, height=1.2in]{figs/new_Visual_HalfCheetah.eps}
% \caption{Velocity change of the HalfCheetah agent in the test tasks with different goal velocities, where the agent adopts Option 1 (blue) and 2 (orange) when increasing and decreasing the speed, respectively.}
% \label{fig:8} 
% \end{figure}

\subsection{Ablation Study}
In this part, we proceed to show the effectiveness of the imitation learning and context-based multi-task learning components of our algorithm through an ablation study. We propose two ablated versions of our algorithm: (1) \textbf{MH-GAIL} -- a variant by replacing the AIRL component of MH-AIRL with GAIL \cite{DBLP:conf/nips/HoE16} (another commonly-used IL algorithm), of which the details are in Appendix \ref{mh-gail}. (2) \textbf{H-AIRL} -- a version that does not consider the task context $C$, which means $P_{\psi}$ (i.e., the variational posterior for $C$) is not adopted, $L^{MI}$ is eliminated from the overall objective (Equation \ref{equ:19}), and other networks do not use $C$ as part of the input. H-AIRL can be viewed as a newly-proposed Hierarchical IL (HIL) algorithm since it integrates the option framework and IL. To be more convincing, we additionally use two SOTA HIL algorithms -- \textbf{Option-GAIL} \cite{DBLP:conf/icml/JingH0MKGL21} and \textbf{DI-GAIL} \cite{DBLP:conf/iclr/SharmaSRK19}, as the baselines. Note that the training with the HIL algorithms are also based on a mixture of multi-task expert data.

% These HIL algorithms do not adopt the context-based multi-task learning component, so they can only learn a single average policy for the class of tasks from the mixture of multi-task demonstrations.

In Appendix \ref{ab-plots}, we provide the plots of the change of episodic rewards on the test tasks in the training process for each algorithm on each evaluation task. The training with each algorithm is repeated for 5 times with different random seeds. We compute the average episodic reward after the learning converges for each algorithm in the 5 runs, and record the mean and standard deviation of them in Table \ref{table:1} as the convergence performance. First, we can see that our algorithm performs the best on all the baselines, which shows the effectiveness of all the main modules of our algorithm. Second, MH-GAIL has better performance than the HIL baselines, showing the necessity to include the context-based multi-task learning component. Without this component, the HIL algorithms can only learn an average policy for the class of tasks from the mixture of multi-task demonstrations. Last, H-AIRL, the newly-proposed HIL algorithm, performs better than the SOTA HIL baselines (i.e., Option-GAIL and DI-GAIL) on the Mujoco tasks.
% Moreover, we can see from Figure \ref{fig:4} that MH-GAIL has better convergence performance than the MIL baselines (i.e., PEMIRL, SMILE, and MAML-IL) on the more challenging Ant \& Kitchen tasks.

\subsection{Analysis on the Learned Hierarchical Policy}
Real-life (robotic) tasks are usually compositional and long-horizontal. Capturing the subtask structures in those tasks can be essential for the (multi-task) policy learning with the reasons: (1) It's more natural and human-like to split a complex task into more manageable subtasks to learn separately and then synthesize these skills to complete the whole task. (2) In some circumstances, the basic skills learned from one task setting can be reused in other task settings so the agent only needs to update its high-level policy accordingly, which significantly lowers the difficulty of multi-task learning. We test our algorithm on Mujoco-MultiGoal (Figure \ref{fig:6(a)}) where the agent is required to achieve a goal corresponding to the task context variable (2-dim Gaussian). The given expert demonstrations for training include 100 goal locations in the Cell and the expert agent goes only moves horizontally or vertically. We test the learned hierarchical policy on 8 sparsely distributed goal locations, of which the trajectories are shown as Figure \ref{fig:6(d)}. We can see: (1) Four options (labeled with different colors) are discovered based on the demonstrations, each of which corresponds to a particular forward direction (green: up, yellow: down, etc.). (2) The agent knows how and when to switch among the options to complete the tasks in stages (i.e., horizontal and vertical) with the learned high-level policy. Moreover, we randomly select 6 task contexts for HalfCheetah-MultiVel and visualize the recovered hierarchical policy as the velocity change of each episode in Figure \ref{fig:7(a)}. It can be observed that the agent automatically discovers two options (Option 1: blue, Option 2: orange) and adopts Option 1 for the acceleration phase ($0 \rightarrow v/2$ or $0 \rightarrow v$) and Option 2 for the deceleration phase ($v/2 \rightarrow 0$). Thus, our algorithm can capture the compositional structure within the tasks very well and take advantage of it in the multi-task policy learning, which explains its superior performance compared with the Meta IL baselines.

Next, previous Meta/Multi-task Learning algorithms can learn a policy for a class of tasks whose contexts follow a certain distribution, but the learned policy cannot be transferred as a whole to tasks out of this class. While, our algorithm recovers a hierarchical policy, of which the low-level part can be reused as basic skills in tasks within similar scenarios but not limited to the task class, which enhances the transferability of the learned policy. To show this, we reuse the options discovered in PointCell as the initialization of the low-level part of the hierarchical policy for the goal-achieving tasks in new scenarios -- PointRoom and PointMaze (Figure \ref{fig:6(b)} and \ref{fig:6(c)}). In each scenario, we select 4 challenging goals (starting from the center point) for evaluation, which are labeled as red points in the figure. Unlike the other evaluation tasks, we provide the agent sparse reward signals (only positive rewards for reaching the goal) instead of expert data, so they are RL rather than IL tasks. We use HPPO proposed in Section \ref{frame} as the Hierarchical RL (HRL) algorithm and initialize it with the transferred options (i.e., HPPO-init). To be more convincing, we use two other SOTA HRL and RL algorithms -- \textbf{DAC} \cite{DBLP:conf/nips/ZhangW19a} and \textbf{PPO} \cite{DBLP:journals/corr/SchulmanWDRK17}, as baselines. In Figure \ref{fig:6(e)} and \ref{fig:6(f)}, we plot the episodic reward change in the training process of each algorithm, where the solid line and shadow represent the mean and standard deviation of the performance across the 4 different goals in each scenario. We can see that the reuse of options significantly accelerate the learning process and the newly proposed HRL algorithm performs much better than the baselines. Note that the other algorithms are trained for more episodes since they do not adopt the transferred options. We show that, in scenarios for which we do not have expert data or dense rewards, we can make use of the basic skills learned from expert demonstrations for similar task scenarios to effectively aid the learning, which provides a manner to bridge IL and RL.

Finally, we note that, for some circumstances, the basic skills need to be conditioned on the task context. For the Mujoco-MultiGoal/MultiVel tasks, the basic skills (e.g., Option 2: decreasing the velocity) can be directly transferred among the tasks in the class and the agent only needs to adjust its high-level policy according to the task variable (e.g., adopting Option 2 when achieving $v/2$). However, for tasks like Walker-RandParam, the skills need to adapt to the task, since the mass of the agent changes and so do the dynamics. As shown in Figure \ref{fig:7(b)},  the learning performance would drop without conditioning the low-level policy (i.e., option) on the task context, i.e., MH-AIRL-no-cnt.

